Fast Planning Over Roadmaps via Selective Densification

We propose the Selective Densification method for fast motion planning through configuration space. We create a sequence of roadmaps by iteratively adding configurations. We organize these roadmaps into layers and add edges between identical configurations between layers. We find a path using best-first search, guided by our proposed estimate of remaining planning time. This estimate prefers to expand nodes closer to the goal and nodes on sparser layers. We present proofs of the path quality and maximum depth of nodes expanded using our proposed graph and heuristic. We also present experiments comparing Selective Densification to bidirectional RRT-connect, as well as many graph search approaches. In difficult environments that require exploration on the dense layers we find Selective Densification finds solutions faster than all other approaches.

==> inputs/approach_with_lemur.tex <==
% !TEX root = ../main.tex

\section{Approach: Selective Densification}
\label{sec:approach}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth, trim={3cm 0 4cm 0},clip]{img/SD_2d_grid.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth, trim={4cm 0 3cm 0},clip]{img/SD_2d_halton_morespacing.png}
    \end{subfigure}
    \caption{Layered Graphs in a 2D C-space using a grid structure (left) and halton sequence (right)}
    \label{fig:2dLayeredGraph}
\end{figure}




Our approaches consists of finding a path on a graph with an embedding into C-space.
The core innovation is the combination of graph structure with a heuristically guided search that balances execution cost and expected remaining planning cost.
The graph has connected layers of different densities allowing the search to traverse to denser layers to navigate through tight spaces with precision and then return to sparser layers that are searched more quickly.
The graph is explored in a Best-Utility-First search, explicitly considering both path cost and planning cost.
As the true remaining planning cost is unknown, it is estimated via a heuristic that grows as the layer depth increases.

%In our approach we add new edges to the original $\graph$, and thus potentially produce a $\path$ not represented in the original graph.
\subsection{Graph Structure}
%Graph $\graph$ is constructed in layers, where each layer is a R-Disk graph.
Consider a sequence of unique configurations $Q = (q_1, q_2, \dots)$, and a strictly increasing sequence positive integers $(n_1 < n_2 < ... n_d)$.
A layer $L_i$ is an $r$-disk graph constructed from the first $n_i$ configurations of $Q$ and connection radius $r_i$.
Denote the vertices of $L_i$ as $v^i_j$ where $j\leq n_i$.
%Note that the configurations represented by the vertices of layer $L_{i+1}$ are a strict superset of those of $L_i$.
For each pair of adjacent layers $(L_i, L_{i+1})$ define the inter-layer edges as $\edges_{i \leftrightarrow i+1} = \{e(v^i_j \leftrightarrow v^{i+1}_j) \  \forall j \leq n_i \}$.
Note that $v^i_j$ and $v^{i+1}_j$ represent the same configuration $q_j$, thus the inter-layer edges are zero-cost edges that change layers without changing configurations.
The Layered Graph is defined as $\graph = (\union_i L_i) \union (\union \edges_{i \leftrightarrow i+1})$.

Figure \ref{fig:2dLayeredGraph} visualizes two Layered Graphs in a 2D C-space, with the vertical dimension representing layer depth.
Vertical edges are therefore the zero-cost edges connecting vertices in adjacent layers representing the same configuration.



A query may consist of a $q_s$ and $q_g$ not represented by $\graph$, thus during a query vertices for $q_s$ and $q_g$ are added to each layer, edges within each $L_i$ are added determined by the connection radius $r_i$, and inter-layer edges are added for the vertices corresponding to $q_s$ and $q_g$.






\subsection{Graph Construction}
The Layered Graph can be constructed explicitly before a query is received, implicitly as nodes are expanded, or a combination of explicit and implicit. 

Explicit construction can remove significant computational burden from the online query.
Naive construction of the $r$-disk graph involves finding all node pairs within the connection distance $r$, and even when storing configurations in a KD tree this can consume significant computation time for large graphs.
Furthermore, certain properties of edges can be precomputed and recalled quickly during query time.
Specifically examined in this work, one such useful property of an edge is the swept volume in the robot workspace.
This allows for faster collision checks between a robot and workspace obstacles for an edge.

Implicit construction has the potential to perform significant densification in a small region without the overhead of computing all nodes and edges for these denser layers.
However, in order for implicit construction to be computationally effective we conjecture the underlying sequence of configurations $Q$ must have a structure that can be exploited to efficiently compute neighbors.
One such sequence with this structure represents grids whose edge-distance halves with each layer depth.

In practice layers can be precomputed depending on available computer memory.
If an exploitable structure exists new nodes can be added implicitly when expanded, or the depth can be limited.









\begin{algorithm}
\caption{Selective Densification Search} \label{alg:lazysp}
\begin{algorithmic}[1]
\While{True}
\State $\path \leftarrow $BestUtilityFirst$(\graph, v_s, v_g)$ \label{alg:lazysp:bestfirst}
\If{CheckEdges($\path$)}
\State \textbf{return} $\path$ 
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Bidirectioanl Selective Densification Search} \label{alg:bilazysp}
\begin{algorithmic}[1]
\State $t_{forward} \leftarrow 0$
\State $t_{backward} \leftarrow 0$
\While{True}
\If{forward\_time $\leq$ backward\_time}
\State $\path \leftarrow $BestUtilityFirst$(\graph, v_s, v_g)$ \label{alg:bilazysp:forward}
\State $t_{forward} \leftarrow t_{forward} +$ timeOf(Line \ref{alg:bilazysp:forward})
\Else
\State $\path \leftarrow $BestUtilityFirst$(\graph, v_g, v_s)$.reverse()
\label{alg:bilazysp:backward}
\State $t_{backward} \leftarrow t_{backward} +$ timeOf(Line \ref{alg:bilazysp:backward})
\EndIf
 \label{alg:bilazysp:bestfirst}
\If{CheckEdges($\path$)}
\State \textbf{return} $\path$ 
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{CheckEdges($\path$)} \label{alg:checkedges}
\begin{algorithmic}[1]
\For{$edge$ in $\path$}
\If{$edge$ is not valid} \label{alg:checkedges:collisioncheck}
\State mark $edge$ as $invalid$
\State \textbf{return} False
\EndIf
\State mark $edge$ as $valid$
\EndFor
\State \textbf{return} True
\end{algorithmic}
\end{algorithm}















\begin{algorithm}
\caption{BestUtilityFirst($\graph, v_s, v_g$)} \label{alg:bestfirst}
\begin{algorithmic}[1]
\State $open \leftarrow \{v_s\}, closed \leftarrow \{\}$
\While{$open$ is not empty}
\State $n \leftarrow open$.pop\_lowest\_$f$value()
\State $closed$.add($n$)
\If{$n$ is $v_g$}
\State \textbf{return} ReconstructPath($v_s, v_g$)
\EndIf
\For{edge $e$ and child $c$ of $n$}
\If{$e$ is $invalid$} skip
\EndIf
\State $g\_temp = g(n) + x(e) + p(e)$ \label{alg:bestfirst:gvalue}
\If{$c$ in $closed$ and $g\_temp < g(n)$}
\State $g(c) \leftarrow g\_temp$
\Else
\State $g(c) \leftarrow g\_temp$
\State $f(c) \leftarrow g(c) + \hat{x}(c) + \hat{p}(c)$ \label{alg:bestfirst:hvalue}
\State $open$.add($c$)
\EndIf
\EndFor
\EndWhile
\State \textbf{return} No Path Exists
\end{algorithmic}
\end{algorithm}



\subsection{Utility Guided Graph Search}

To answer a query $(q_s, q_g)$ first the corresponding graph nodes $(v_s, v_g)$ are found, a best-first search with lazy edge-evaluation is performed over the graph yielding a path through $\graph$, and the induced C-space path is returned.

Algorithms \ref{alg:lazysp} and \ref{alg:checkedges} show the outer-most loops that perform the lazy edge evaluation.
Line \ref{alg:lazysp:bestfirst} of Alg. \ref{alg:lazysp} performs a best-first search under the optimistic assumption that unevaluated edges are collision free.
Edges along this optimistic path are collision-checked by Alg. \ref{alg:checkedges}.
The result of a collision check is stored so that future iterations of the best-first search may not traverse invalid edges.


The BestUtilityFirst search algorithm is shown in Alg. \ref{alg:bestfirst} and is identical to A$^*$ with modified $g$ and $h$ values, or cost-to-come and estimated cost-to-go.
BestUtilityFirst requires four functions: The execution cost for an edge $\executioncost(e)$, the planning cost for an edge $\planningcost(e)$, a heuristic estimate of execution cost-to-go $\hat{\executioncost}(v)$ and a heuristic estimate of planning cost-to-go $\hat{\planningcost}(v)$.
A temporary $g$ value for a child node is calculated in line \ref{alg:bestfirst:gvalue} using the $g$ value of the parent, and the total cost for an edge, $\executioncost(e) + \planningcost(e)$.
The $f$ value in line $\ref{alg:bestfirst:hvalue}$ determines the priority of node expansion by summing the $g$ value with a heuristic estimate of remaining cost-to-go, $\hat{\executioncost}(v) + \hat{\planningcost}(v)$. 


%The Best-First search in Alg. \ref{alg:lazysp} Line \ref{alg:lazysp:bestfirst} could be implemented via any one of many different graph search methods over $\graph$.
%Graph search methods, such as Dijkstra's or A$^*$ with an admissible heuristic obtain the path of lowest execution cost but do not consider planning time and therefore may yield solutions with low utility due to increased planning cost.
%Specifically for a Layered Graph optimal graph search methods lack an incentive to explore the sparser layers for which planning cost is significantly cheaper.

BestUtilityFirst can be viewed as combining the approaches of BUGSY \cite{Ruml2007} and LEMUR \cite{Dellin2016}, and perform an A$^*$ search with modified $g$ and $h$.
The cost-to-come to a node, or $g$ values are modified to include the remaining planning time required to evaluate the path to a node, in addition to standard execution cost to the node.
The heuristic cost-to-go, or $h$ values are modified to include an estimate of the remaining planning cost as well as execution cost.

\subsection{Cost Functions} \label{sec:PlanningHeuristic}
We now define and explain the four cost functions used in BestFirstUtility: $\executioncost, \hat{\executioncost}, \planningcost, \hat{\planningcost}$.

The execution cost $\executioncost$ and heuristic $\hat{\executioncost}$ are the same as in many robotic graph search problems.
For this work we use the path length as execution cost $\executioncost(e) = w_x ||q_1 - q_2||$ where $q_1$ and $q_2$ are the configuration at the edge endpoints and $w_x$ is given in the provided utility function $\utility$, and defines the weight of the execution cost as part of the total cost.

We estimate the remaining execution cost at a vertex via the admissible heuristic $\hat{\executioncost}(v_1) = w_x || q_1 - q_g||$ where $q_1$ is the configuration at $v_1$ and $q_g$ is the goal configuration.
Other execution costs may also be used with this core algorithm, so long as the the total execution cost can be represented as the sum of edge execution costs.

The planning cost of an edge $\planningcost(e)$ represents the remaining computational cost of evaluating a path through $e$.
$\planningcost$ prioritizes expansion of edges with known validity for nodes with otherwise similar $f$values because this saves evaluation time.
We approximate $\planningcost$ by assuming the remaining planning cost is dominated by the collision-checking for unevaluated edges.
For an edge with known validity, $\planningcost(e) = 0$.
With unknown validity, $\planningcost(e)$ is the estimated time to collision-check the edge.
We set $\planningcost(e) = w_p t_{cc} \frac{||q_1 - q_2||}{d}$, where $w_p$ is provided by the utility function $\utility$, $t_{cc}$ is the time to collision-check a configuration, $q_1$ and $q_2$ are the edge endpoints, and $d$ is the discretization distance.
In practice the true time to collision-check an edge may be lower, as if a collision is found the remaining configurations do not need to be checked.



%We approximate $p(e)$ assuming the primary computation cost is the collision-check of an edge.
%For an edge with known validity $p(e) = 0$. 
%For an edge with unknown validity we set $p(e)$ as the estimated computation time of determining the validity.
%This is at most the time per configuration-check multiplied by the number of discrtized configurations along an edge.

%The heuristic value is used in Line $\ref{alg:bestfirst:hvalue}$, where $\hat{\executioncost}$ is the heuristic execution cost and $\hat{\planningcost}$ is the heuristic planning cost to reach the goal.
%The combination of $\hat{\executioncost}$ and $\hat{\planningcost}$ guides the search towards nodes that have low
%The form of the heuristic used is discussed in the next section.

The planning cost-to-go heuristic $\hat{\planningcost}$ guides search towards vertices that likely require little planning cost to reach the goal.
As denser layers of our graph require more time to search, $\hat{\planningcost}$ incentivizes search of sparser layers first.

Again we assume the dominant planning cost is due to collision-checks, and therefore estimate the remaining planning cost-to-go for a vertex $v$ by approximating the number of configurations that will require collision-checks between $v$ and the goal $v_g$.
The true number of configuration collision-checks is unknown, and may vary wildly.
As a lower bound, during a particular run of BestUtilityFirst it is possible that all edges along a path between $v$ and $v_g$ have been checked in previous iterations, thus no edges require future checks.
However in the pathological case, there may be only one collision free path and this path is evaluated last, thus a complete search from $v$ may require evaluation of every edge on the graph.




%We tailor this estimate towards ``hard" environments with misleading paths where all edges within a volume are collision-checked before the A$^*$ search "escapes".
%Furthermore we estimate $\hat{p}$ at a particular layer assuming the remainder of the search continues on the same layer

It has been found that environments challenging for motion planning algorithms may contain regions sometimes called ``bug traps" or ``cul-de-sacs" that mislead a heuristic and require significant search effort to escape \cite{PlanningAlgorithms}.
For a search of $\graph$, such a region $\mathcal{R} \subset \cspace$ may require evaluation of all edges on a layer $i$ that contain an endpoint configuration within  $\mathcal{R}$.

We set 
\begin{align}\hat{p}(v_1) = w_p n_i c_p ||q_1 - q_g||\end{align}
where $v_1$ in in layer $i$, $n_i$ is the number of nodes in layer $i$, $q_1$ and $q_g$ are the configurations of $v_1$ and the goal, and $c_p$ is a tunable constant.
Note that we construct graphs such that $|\edges_i| \sim n_i$, thus $\hat{\planningcost} \sim |\edges_i|$.


The effect of these cost functions can be seen in Figure \ref{fig:2dSearch} and Figure \ref{fig:culdesac}.
In Figure \ref{fig:2dSearch} the search explores the sparest edge in the top layer but neither is valid.
The search progresses to denser layers in the regions closest to the goal.
In this example the search only progresses to the level of densification necessary, and only in regions closer to the goal.
Although the graph extends deep, these edges are never explored.
Note that without a planning heuristic the search would immediately explore edges on the most dense layer, as these nodes have the lowest $x(e) + p(e) + \hat{x}(v)$ values.

Figure \ref{fig:culdesac} demonstrates the behavior in a cul-de-sac, created by the region in the upper right that is close to but blocked off from the goal.
Based on the heuristic estimate the upper right region appears close to the goal.
Selective Densification explores the sparser layers in this trap and finds no valid edges.
The planning heuristic adds cost to deeper layers and therefore encourages breadth.
Both the planning heuristic and execution heuristic guide the search to nodes close to the goal.
Once the search passes the narrow gaps the longer edges on the sparer layers have the lowest total $f$-value, allowing the search to reach the goal with little search effort.



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\textwidth]{img/SD_2d_overview.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\textwidth]{img/SD_2d_grid_side_search_edges.png}
    \end{subfigure}
    \caption{A 2D search problem solved using Selective Densification with evaluated edges shown in black (valid) and red (invalid) and the final path shown in blue. Top: 2D view with red obstacles. Bottom: View of Layered Graph with unevaluated edges shown in light-grey}
    \label{fig:2dSearch}
\end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\textwidth]{img/cul_de_sac.png}
    \end{subfigure}
    \hfill

    \caption{Selective Densification search with a misleading trap. Dense nodes are expanded near the goal where the cost-to-come plus estimated cost-to-go are low. Sparse layers have lower planning cost estimates, encouraging a mixture of depth and breadth in the search.}
    \label{fig:culdesac}
\end{figure}






==> inputs/implementation.tex <==
% !TEX root = ../main.tex

\section{Implementation}
\label{sec:implementation}

We implemented Selective Densification in C++.
Robot-environment collision checking used GPU-Voxels \cite{Hermann2014} with a voxel grid of 200x200x200 and a voxel size of 2cm$^3$.
Collision checks were performed by intersecting the voxel grid representing the robot with the voxel grid representing the environment obstacles.
A NVidia 1080Ti GPU and an Intel i7-7700K CPU was used for all experiments.
A single collision check took approximately $1ms$.

\subsection{Halton Graph Creation}
For experiments we implemented a 16-Layered Graph using $Q$ as a 7D halton sequence, the number of nodes in layer $i$ was $n_i = 2^i$, and the connection radius at each layer $r_i$ was set so the expected number of edges per node is 30, consistent with previous halton roadmap experiments \cite{LazySP}.

\subsection{Optimizations}
Collision-checking of edge $e$ is implemented by checking discretized configurations $q_1, q_2,...$.
These configurations are checked in a random order, which tends to discover invalid configurations (and therefore invalid edges) faster than checking by proceeding along the edge.

%Since collision checking is expensive relative to graph search, we search using the generalized version of LazyPRM, LazySP \cite{lazysp}. 
%A* queries a path through the graph under the optimistic assumption that unchecked edges are collision free, then collision-check edges along this path until an invalid edge is encountered, or the goal is reached.
%This processes is repeated until no invalid edge is found along the path.

%% As bidirectional approaches tend to perform faster than single direction searches, we alternate the BestFirst searches from the start-to-goal and goal-to-start in Alg. \ref{alg:lazysp} Line \ref{alg:lazysp:bestfirst}, creating a bidirectional search. 
%% We considered two alternative bidirectional approaches.
%% We first tried alternating between forward and backward searches at each iteration.
%% We also tried balancing the total time between forward and backward searches.

%Note that since the A* heuristic used is inadmissible the path found via forward and reverse searches may differ, thus this approach is distinct from an alternating edge-selector.


\subsection{Precomputing and Caching Swept Volumes}
When collisions are caused by overlap between the robot and workspace obstacles, edge validity can also be determined by checking for overlap between the swept volume of discretized configurations along an edge with obstacles in the environment. 
The swept volumes can be precomputed for some $e \in \edges$, and a collision check can be performed via a lookup of the swept volume followed by an intersection with the environment.

